HZ Recoil Mass and Cross Section Analysis in ILD

This note describes the details of a simulation study of the Higgs boson production for processes in which the Higgs is produced together with a well measurable di-lepton system using the proposal of the ILD detector for its Letter of Intent. The analysis is optimised for the measurement of the Higgs-strahlung process, i.e. e+e- -> HZ. The cross section can be determined with a precision of 2-3% and by combining the decay channels a precision of ~30 MeV is obtained for the mass of the Higgs boson. The background can be largely reduced and the analysis exhibits a sensitivity to the configuration of the accelerator.

==> gammagamma/gammagamma.tex <==
Radiative effects on the incoming beam lead to a considerable fraction to interactions between the 
radiated photons. Being a pure QED process the background induced by 
$\gamma\gamma\rightarrow\epem\mpmm$, has a cross section which is several orders of magnitude higher than 
that of the Higgs-Strahlungs process. A safe rejection of this background requires an efficient identification of the
deflected beam electrons which is particularly true for the $\gamma\gamma\rightarrow\epem$ process. 

This section introduces  means to the $\gamma\gamma$ background to the Higgs-Strahlung process in which the
$\Zzero$-Boson decays leptonically. Here only processed in which both photons are on mass shell are considered.

 \section*{Pre-selection}
The large cross section of $\gamma\gamma$ scattering, see also Tables~\ref{crossSectionEE} and~\ref{crossSectionMM}, 
requires a preselection of the generated events before these are subject to the simulation and reconstruction steps. 
The selection criteria are as follows:

Pre-selection cuts for $\gamma\gamma\rightarrow\epem$:
\begin{itemize}
 \item $N_egood > $ 2
\end{itemize}
or
\begin{itemize}
 \item $N_{e,good} = $ 2
 \item $\sum P_t > $ 10 GeV/c
 \item $M_{e^+e^-} > $ 60 GeV/c$^2$
\end{itemize}
Here $N_{e,good}$ is the number of electrons or positrons in the range of
$|\cos\theta | < 0.95$. Table \ref{crossSectionEE} shows the cross sections of $\epem\rightarrow\Zzero\Higgs\rightarrow\eplus\eminus X$ 
and $\gamma\gamma\rightarrow ee$ for the polarisation mode $\eminus_L\eplus_R$. The cross section after the pre-selection is indicated in parentheses.

\begin{table}[htbp]
 \begin{center}
  \begin{tabular}[tb]{|l|l|}
   \hline
   processes& cross section \\\hline
   $ZH\rightarrow eeX$& 11.107 fb\\ \hline
   $\gamma\gamma\rightarrow ee$& 2.602 nb (19.29 pb)\\ \hline
  \end{tabular}
  \caption{
  Cross sections for the $eeX$-channel for the polarisation mode $\eminus_L\eplus_R$.
  }
  \label{crossSectionEE}
 \end{center}
\end{table}

Pre-selection cuts for $\gamma\gamma\rightarrow\mpmm$:
\begin{itemize}
 \item $\sum P_t > $ 10\,GeV
\end{itemize}
\begin{table}[htbp]
 \begin{center}
  \begin{tabular}[tb]{|l|l|}
   \hline
   processes& cross section \\\hline
   $ZH\rightarrow \mu\mu X$& 10.4026 fb\\ \hline
   $\gamma\gamma\rightarrow \mu\mu$& 2.602 nb (427 fb)\\ \hline
  \end{tabular}
  \caption{Cross sections for $\mu\mu X$ channel for the polarisation mode $\eminus_L\eplus_R$.}
  \label{crossSectionMM}
 \end{center}
\end{table}

Table~\ref{crossSectionMM} shows the cross
sections of $\epem\rightarrow\Zzero\Higgs\rightarrow\mpmm X$ and $\gamma\gamma\rightarrow\mpmm$ for
the polarisation mode $\eminus_L\eplus_R$. The cross section after the pre-selection is indicated in parentheses.

\section*{Rejection of $\gamma\gamma$ background}
%\subsection{Normal cuts}
On the simulated the following cuts are initially applied, called \emph{Normal Cuts} hereafter;
\begin{itemize}
 \item $115< M_{recoil} <150$\,GeV
 \item $80 < M_{Z} <100$\,GeV
 \item $P_t^{di-lepton} > $ 20\,GeV
 \item $0.2<Acoplanarity< 3$\,rad
\end{itemize}
These cuts are similar to those introduced in~\ref{sec:sigbak}.

Table \ref{normalCutEE} and Table \ref{normalCutMM}
show the number of events after applying the \emph{Normal Cuts} for the $ee X$-channel 
and the $\mu\mu X$-channel, respectively.

%For electron channel, since the number of events of the gamma-gamma background
%is still large, some more cuts are needed.
%On the other hand, additional cut is not needed for muon channel.

%We report more rejection cuts for electron channel in the following sections.

\begin{table}[htbp]
 \begin{center}
  \begin{tabular}[tb]{|l|l|l|}
   \hline
   & $ZH\rightarrow eeX$& $\gamma\gamma\rightarrow
   ee$\\\hline
   no cut& 2777& 650M\\ \hline
   + pre-selections& 2777 (100\%) & 4.69M (0.721\%)\\ \hline
   + normal cuts& 1380 (49.68\%)& 5365 (8.25$\times10^{-6}$)\\ \hline
  \end{tabular}
  \caption{Reduction rate for electron channel with polarization $e_L^-e_R^+$, total integrated luminosity of 250 fb$^{-1}$.}
  \label{normalCutEE}
 \end{center}
\end{table}

\begin{table}[htbp]
 \begin{center}
  \begin{tabular}[tb]{|l|l|l|}
   \hline
   & $ZH\rightarrow \mu\mu X$& $\gamma\gamma\rightarrow
   \mu\mu$\\\hline
   no cut& 2601& 650M\\ \hline
   + pre-selections& 2601 (100\%) & 0.104M (0.02\%)\\ \hline
   + normal cuts& 1381 (53.1\%)& 14.6 (2.25$\times10^{-8}$)\\ \hline
  \end{tabular}
  \caption{Reduction rate for muon channel with polarization $e_L^-e_R^+$, total integrated luminosity of 250 fb$^{-1}$.}
  \label{normalCutMM}
 \end{center}
\end{table}

\subsection*{Hits on BeamCal}
While the cuts introduced in the previous section a sufficient to reject events in which muon pairs are 
produced, they have to be extended for the case of electron pairs in the final state of the $\gamma\gamma$ scattering. 
Signal in the BeamCal located close to the beam pipe can be used to identify deflected beam 
electrons or positrons. In the simulated sample the crossing angle of 14\,mrad is not taking into account.
Therefore the particle trajectory is calculated from the generator information and extrapolated to the corrected 
BeamCal position. Events in which a beam particle deposits more than 40\,GeV in the BeamCal are rejected.
  
\subsection*{The Polar angle of the $\Zzero$ decay products}
\emph{ Original text: Z boson is uniformly decays into electron pairs in the rest frame of
it. {\bf RP: Is this really true??? Forward Backward Asymmetry!!!}The distribution of $\cos\theta$ in the rest frame of Z boson was
checked (Figure \ref{cos}, \ref{cosAA}), where we assigned the flight direction of Z boson to z-axis.
The events in the range of $|\cos\theta|<0.8$ are selected.}

If the invariant mass of a di-lepton pair yields the mass of the $\Zzero$-Boson the polar angle distribution of the
tentative decay products is calculated in the rest frame of the $\Zzero$ Boson. For the boost it is assumed that the $\Zzero$-Boson
moves into the direction of the positive $z$-axis, thus the electron flight direction. The Figures~\ref{cos} and~\ref{cosAA} shows the
polar angle distribution of the di-lepton pair where each of the two particles leads to an individual entry. It is clearly visible that the
leptons  created by $\gamma\gamma$ scattering do have a different polar angle distribution. This motivates a cut on $|\cos\theta|<0.8$ to reject events from the $\gamma\gamma$ background.

\begin{figure}[htbp]
 \begin{tabular}[tb]{cc}
  \begin{minipage}[cbt]{0.5\hsize}
   \begin{center}
    \includegraphics[width=\hsize]{ncos.eps}
    \caption{The distribution of $\cos\theta$ in the rest frame of Z
    boson for signal. Z boson is uniformly decays into electron pairs
    in the rest frame of it.}
    \label{cos}
   \end{center}
  \end{minipage}
  \begin{minipage}[cbt]{0.5\hsize}
   \begin{center}
    \includegraphics[width=\hsize]{ncos_aa.eps}
    \caption{The distribution of $\cos\theta$ in the rest frame of Z
    boson for gamma-gamma background.}
    \label{cosAA}
   \end{center}
  \end{minipage}
 \end{tabular}
\end{figure}

\subsection*{$\cos\theta$ in the lab frame}
Figure \ref{ncosLab}-\ref{pcosLabAA} show the distribution of $\cos\theta$ of the electron or positron in the laboratory  frame, $\cos\theta_{lab}$. As expected the distributions increase strongly towards $|\cos\theta_{lab}|=1$ for $\gamma\gamma$ background events since
these entries are generated by deflected beam particles. In case of the Higgs-Strahlung events the final state leptons are distributed
approximatively equal within the range $-1<\cos\theta_{lab}<1$ This observation motivates the cuts $\cos\theta_{lab}<0.7$ for electron and
$\cos\theta_{lab}>-0.7$ for final state positrons for the  rejection of events created by $\gamma\gamma$ background.

\begin{figure}[htbp]
 \begin{tabular}[tb]{cc}
  \begin{minipage}[cbt]{0.5\hsize}
   \begin{center}
    \includegraphics[width=\hsize]{ncosLab.eps}
    \caption{The distribution of $\cos\theta$ of electron in the lab frame
   for signal.}
    \label{ncosLab}
   \end{center}
  \end{minipage}
  \begin{minipage}[cbt]{0.5\hsize}
   \begin{center}
    \includegraphics[width=\hsize]{ncosLab_aa.eps}
    \caption{The distribution of $\cos\theta$ of electron in the lab frame
   for gamma-gamma background.}
   \end{center}
  \end{minipage}
 \end{tabular}

\begin{tabular}[tb]{cc}
\begin{minipage}[cbt]{0.5\hsize}
   \begin{center}
  \includegraphics[width=\hsize]{pcosLab.eps}
    \caption{The distribution of $\cos\theta$ of positron in the lab frame
   for signal.}
 \end{center}
\end{minipage}
\begin{minipage}[cbt]{0.5\hsize}
   \begin{center}
  \includegraphics[width=\hsize]{pcosLab_aa.eps}
    \caption{The distribution of $\cos\theta$ of positron in the lab frame
   for gamma-gamma background.}
    \label{pcosLabAA}
 \end{center}
\end{minipage}
\end{tabular}
\end{figure}

\section*{Reduction rate}
Table \ref{reductionAll} shows the reduction rate for electron channel.
The gamma-gamma background ($\gamma\gamma\rightarrow\eplus\eminus$) produced by the scattering of real photons  is nearly completely rejected. The cuts introduced here need however to be synchronised with the ones introduced in the main text. Additionally,
The background rate for virtual photon scattering has still to be estimated. Finally, the results presented here have to be confirmed by a study which includes an adequate simulation of the crossing angle and the BeamCal. 


\begin{table}[htbp]
 \begin{center}
  \begin{tabular}[tb]{|l|l|l|}
   \hline
   & $ZH\rightarrow eeX$& $\gamma\gamma\rightarrow
   ee$\\\hline
   no cut& 2777& 650M\\ \hline
   + pre-selections& 2777 (100\%) & 4.69M (0.721\%)\\ \hline
   + normal cuts& 1380 (49.68\%)& 5365 (8.25$\times10^{-6}$)\\ \hline
   + Hits on BeamCal& 1378 (49.62\%)& 4591 (7.06$\times10^{-6}$)\\ \hline
   + $|\cos\theta|<0.8$& 1148 (41.34\%)& 2301 (3.54$\times10^{-6}$)\\ \hline
   + $\cos\theta_{lab}<0.7$& 753 (27.1\%)&24 (3.72$\times10^{-8}$)\\ \hline
  \end{tabular}
  \caption{Reduction rate for electron channel with polarization
  $e_L^-e_R^+$, total integrated luminosity of 250 fb$^{-1}$.}
  \label{reductionAll}
 \end{center}
\end{table}
%\end{document}



==> reactions.tex <==
%\documentclass[9]{article}


%\usepackage[latin1]{inputenc}
%\usepackage[dvips]{graphicx,epsfig,color}
%\usepackage{wrapfig,rotating}
%\usepackage{amssymb,amsmath,array}
%\pagestyle{empty}

%\pdfpagewidth=29.7cm
%\pdfpageheight=21cm
%\textwidth=29.5cm
%\hoffset=-4.4cm

%\begin{document}





\begin{table}[htdp]
\label{tab:reactionmmx}
\begin{footnotesize}
\caption{Breakdown of statistics of processes used in the analysis for the $\mu\mu X$-channel}
\end{footnotesize}
\centering
\begin{tiny}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline

$Reactions$ & $\sigma_{+-}$ & $\sigma_{-+}$ & $\sigma_{++}$ & $\sigma_{--}$ & $\mathcal{L}$ & $Ns_{+-}$ & $Ns_{-+}$ & $Ns_{++}$ & $Ns_{--}$& $\sigma_{RL}$ & $\sigma_{LR}$ & $N_{RL+-}$ & $N_{RL-+}$ & $N_{RL++}$ & $N_{RL--}$ & $N_{LR+-}$ & $N_{LR-+}$ & $N_{LR++}$ & $N_{LR--}$ \\
\hline
e2e2h & 10.967 & 17.126 & 0 & 0 & 1000 & 10967 & 17126 & 0 & 0 & 7.0151 & 10.4026 & 6415 & 599 & 0 & 0 & 383 & 10018 & 0 & 0 \\ 
\hline
e2e2 & 215.632 & 330.426 & 0 & 0 & 500 & 110216 & 129338 & 0 & 0 & 137.71 & 200.846 & 63072 & 5782 & 0 & 0 & 3773 & 96649 & 0 & 0 \\ 
\hline
e3e3 & 12852.9 & 17102.4 & 0 & 0 & 9 & 98800 & 98800 & 0 & 0 & 8117.53 & 10454.8 & 67670 & 5387 & 0 & 0 & 4048 & 90044 & 0 & 0 \\ 
\hline
e1e1e2e2 & 1088.6 & 1106.71 & 1073.64 & 1073.64 & 150 & 100000 & 100000 & 99400 & 97400 & 1083.55 & 1093.51 & 95524 & 5810 & 50729 & 10467 & 5715 & 97113 & 10467 & 50729 \\ 
\hline
e2e2e2e2 & 7.234 & 11.4311 & 0 & 0 & 1000 & 10000 & 10431 & 0 & 0 & 4.63198 & 6.94038 & 4231 & 400 & 0 & 0 & 253 & 6687 & 0 & 0 \\ 
\hline
e2e2e3e3 & 14.659 & 23.1405 & 0 & 0 & 1000 & 14658 & 23140 & 0 & 0 & 9.38543 & 14.0503 & 8575 & 809 & 0 & 0 & 513 & 13537 & 0 & 0 \\ 
\hline
n2e2e2n2 & 19.3972 & 779.633 & 0 & 0 & 180 & 15797 & 85200 & 0 & 0 & 38.6345 & 456.764 & 2042 & 4911 & 0 & 0 & 122 & 82095 & 0 & 0 \\ 
\hline
n1n1e2e2 & 12.8466 & 44.7068 & 0 & 0 & 1000 & 12847 & 44707 & 0 & 0 & 9.08 & 26.6031 & 7515 & 1564 & 0 & 0 & 449 & 26153 & 0 & 0 \\ 
\hline
n3n3e2e2 & 12.8475 & 24.7238 & 0 & 0 & 1000 & 12447 & 23724 & 0 & 0 & 8.38112 & 14.9131 & 7515 & 865 & 0 & 0 & 449 & 14463 & 0 & 0 \\ 
\hline
e2e2ss & 30.1803 & 57.6073 & 0 & 0 & 1000 & 29980 & 57607 & 0 & 0 & 19.6717 & 34.7566 & 17655 & 2016 & 0 & 0 & 1056 & 33700 & 0 & 0 \\ 
\hline
e2e2dd & 30.2016 & 57.5377 & 0 & 0 & 1000 & 30202 & 56538 & 0 & 0 & 19.6818 & 34.7166 & 17667 & 2013 & 0 & 0 & 1057 & 33659 & 0 & 0 \\ 
\hline
e2e2bb & 29.5793 & 56.5071 & 0 & 0 & 1000 & 28779 & 56307 & 0 & 0 & 19.2816 & 34.0919 & 17303 & 1977 & 0 & 0 & 1035 & 33056 & 0 & 0 \\ 
\hline
cce2e2 & 29.3345 & 53.1354 & 0 & 0 & 1000 & 29335 & 52735 & 0 & 0 & 19.0204 & 32.1109 & 17160 & 1859 & 0 & 0 & 1026 & 31084 & 0 & 0 \\ 
\hline
uue2e2 & 29.2736 & 53.0187 & 0 & 0 & 1000 & 28474 & 41619 & 0 & 0 & 18.9807 & 32.0405 & 17125 & 1855 & 0 & 0 & 1024 & 31015 & 0 & 0 \\ 
\hline

\end{tabular}
\end{tiny}
\label{tab:mu}
\end{table}%

%\begin{tiny}
%The symbols in the columns of the table have the following meaning: 
%\begin{itemize}
%\item $\sigma_{+-,...}, N_{s_{+-},...}$ are the cross sections and the number of events for fully polarized beams where '$+$' the first symbol
%denotes the polarisation of the electron beam while the second one that of the positron beam.
%\item $\mathcal{L}$ denotes the Luminosity used in the analysis.
%\item $\sigma_{RL,...}, N_{RL_{+-},...}$ are the cross sections and the number of events after correcting for the 
%beam polarisation used in the analysis following the equation in~\cite{gudi}, i.e. $RL$: $\eminus: +80\%$ and $\eplus: -30\%$ and $LR$: $\eminus: -80\%$ and $\eplus: +30\%$
%\end{itemize}
%\end{tiny}

\begin{table}[htdp]
\label{tab:reactioneex}
\begin{footnotesize}
\caption{Breakdown of statistics of processes used in the analysis for the $ee X$ channel}
\end{footnotesize}
\centering
\begin{tiny}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline

$Reactions$ & $\sigma_{+-}$ & $\sigma_{-+}$ & $\sigma_{++}$ & $\sigma_{--}$ & $\mathcal{L}$ & $Ns_{+-}$ & $Ns_{-+}$ & $Ns_{++}$ & $Ns_{--}$& $\sigma_{RL}$ & $\sigma_{LR}$ &  $N_{RL+-}$ & $N_{RL-+}$ & $N_{RL++}$ & $N_{RL--}$ & $N_{LR+-}$ & $N_{LR-+}$ & $N_{LR++}$ & $N_{LR--}$ \\
\hline
e1e1h & 11.289 & 17.892 & 0.645 & 0.645 & 1000 & 11289 & 17892 & 10000 & 10000 & 7.47538 & 11.107 & 6604 & 626 & 203 & 41 & 395 & 10466 & 41 & 203 \\ 
\hline
e1e1 & 658.884 & 733.926 & 630.695 & 632.155 & 500 & 266818 & 242305 & 295769 & 284541 & 650.894 & 692.532 & 192723 & 12843 & 99334 & 20545 & 11530 & 214673 & 20497 & 99564 \\ 
\hline
e3e3 & 12852.9 & 17102.4 & 0 & 0 & 9 & 98800 & 98800 & 0 & 0 & 8117.53 & 10454.8 & 67670 & 5387 & 0 & 0 & 4048 & 90044 & 0 & 0 \\ 
\hline
e1e1e2e2 & 1088.6 & 1106.71 & 1073.64 & 1073.64 & 150 & 100000 & 100000 & 99400 & 97400 & 1083.55 & 1093.51 & 95524 & 5810 & 50729 & 10467 & 5715 & 97113 & 10467 & 50729 \\ 
\hline
e1e1e1e1 & 982.404 & 995.595 & 943.694 & 942.464 & 150 & 97800 & 88600 & 98800 & 94200 & 968.076 & 975.023 & 86205 & 5226 & 44589 & 9189 & 5157 & 87363 & 9201 & 44531 \\ 
\hline
e1e1e3e3 & 948.704 & 965.145 & 942.984 & 941.685 & 150 & 100000 & 99600 & 97600 & 98800 & 947.021 & 955.739 & 83248 & 5067 & 44555 & 9181 & 4980 & 84691 & 9194 & 44494 \\ 
\hline
n1e1e1n1 & 27.458 & 939.099 & 43.625 & 43.584 & 180 & 26600 & 99200 & 42025 & 42784 & 65.5062 & 566.899 & 2891 & 5916 & 2473 & 509 & 172 & 98887 & 510 & 2471 \\ 
\hline
n2n2e1e1 & 21.403 & 38.307 & 16.124 & 16.118 & 1000 & 21403 & 38307 & 16124 & 14718 & 19.9882 & 29.2839 & 12520 & 1340 & 5079 & 1047 & 749 & 22409 & 1048 & 5077 \\ 
\hline
n3n3e1e1 & 21.403 & 38.285 & 16.146 & 16.108 & 1000 & 20403 & 37132 & 15146 & 16108 & 19.9937 & 29.2693 & 12520 & 1339 & 5085 & 1047 & 749 & 22396 & 1049 & 5074 \\ 
\hline
e1e1ss & 85.453 & 123.972 & 73.152 & 73.253 & 1000 & 65600 & 99000 & 71752 & 73253 & 82.1333 & 103.344 & 49990 & 4339 & 23042 & 4761 & 2990 & 72523 & 4754 & 23074 \\ 
\hline
e1e1dd & 85.326 & 123.983 & 73.442 & 73.392 & 1000 & 83526 & 98000 & 72442 & 70192 & 82.1598 & 103.409 & 49915 & 4339 & 23134 & 4770 & 2986 & 72530 & 4773 & 23118 \\ 
\hline
e1e1bb & 68.978 & 106.063 & 57.31 & 57.221 & 1000 & 68978 & 114000 & 57310 & 67042 & 65.8363 & 86.2108 & 40352 & 3712 & 18052 & 3719 & 2414 & 62046 & 3725 & 18024 \\ 
\hline
cce1e1 & 464.383 & 506.805 & 448.339 & 448.721 & 325 & 96800 & 92800 & 98600 & 70000 & 459.796 & 483.223 & 88290 & 5764 & 45898 & 9479 & 5282 & 96356 & 9471 & 45937 \\ 
\hline
uue1e1 & 464.733 & 505.705 & 449.636 & 448.519 & 325 & 96200 & 98600 & 96800 & 84800 & 460.358 & 482.613 & 88357 & 5752 & 46031 & 9474 & 5286 & 96147 & 9498 & 45917 \\ 
\hline 


\end{tabular}
\end{tiny}
\label{tab:el}
\end{table}%


%\end{document}

==> results.tex <==
%\documentclass[9]{article}


%\usepackage[latin1]{inputenc}
%\usepackage[dvips]{graphicx,epsfig,color}
%\usepackage{wrapfig,rotating}
%\usepackage{amssymb,amsmath,array}
%\pagestyle{empty}

%\pdfpagewidth=29.7cm
%\pdfpageheight=21cm
%\textwidth=29.5cm
%\hoffset=-4.4cm

%\begin{document}




\begin{table}[!h]
\centering
\begin{tabular}{|l|c|l|l|l|}

\hline
Fit. &	Pol. &	Ch. &	$\mH$ (GeV) &	$\sigma$ (fb) \\ \hline
&	$\eminus_R\eplus_L$ &	$\mu\mu X$ &	119.984	$\pm$	0.090	&	7.11	$\pm$	0.50	(	7.03	\%)	\\ \cline{3-5}
&	$\mathcal{L}=250\ ,\invfb$ &	$eeX$ &	120.046	$\pm$	0.182	&	7.15	$\pm$	0.87	(	12.17	\%)	\\ \cline{3-5}
&	&	merged &	119.996	$\pm$	0.081	&							\\ \cline{2-5}
&	$\eminus_L\eplus_R$ &	$\mu\mu X$ &	119.854	$\pm$	0.085	&	10.54	$\pm$	0.70	(	6.64	\%)	\\ \cline{3-5}
GPET &	$\mathcal{L}=250\ ,\invfb$ &	$eeX$ &	119.922	$\pm$	0.150	&	11.72	$\pm$	1.15	(	9.81	\%)	\\ \cline{3-5}
&	&	merged &	119.871	$\pm$	0.074	&							\\ \cline{2-5}
&	Joined &	$\mu\mu X$ &	119.915	$\pm$	0.087	&							\\ \cline{3-5}
&	$\mathcal{L}=$ $125\,\invfb(\eminus_R\eplus_L)$ &	$eeX$ &	119.972	$\pm$	0.164	&							\\ \cline{3-5}
&	$\ \ \ \ + 125\,\invfb(\eminus_L\eplus_R)$&	merged &	119.928	$\pm$	0.077	&							\\ \hline

&	$\eminus_R\eplus_L$ &	$\mu\mu X$ &	120.086	$\pm$	0.100	&	6.91	$\pm$	0.50	(	7.24	\%)	\\ \cline{3-5}
&	$\mathcal{L}=250\ ,\invfb$ &	$eeX$ &	119.961	$\pm$	0.244	&	7.15	$\pm$	0.87	(	12.17	\%)	\\ \cline{3-5}
&	&	merged &	120.068	$\pm$	0.093	&							\\ \cline{2-5}
&	$\eminus_L\eplus_R$ &	$\mu\mu X$ &	120.078	$\pm$	0.095	&	10.83	$\pm$	0.72	(	6.65	\%)	\\ \cline{3-5}
CEG &	$\mathcal{L}=250\ ,\invfb$ &	$eeX$ &	120.007	$\pm$	0.185	&	11.75	$\pm$	1.15	(	9.79	\%)	\\ \cline{3-5}
&	&	merged &	120.063	$\pm$	0.085	&							\\ \cline{2-5}
&	Joined &	$\mu\mu X$ &	120.082	$\pm$	0.097	&							\\ \cline{3-5}
&	$\mathcal{L}=$ $125\ ,\invfb(\eminus_R\eplus_L)$ &	$eeX$ &	119.990	$\pm$	0.208	&							\\ \cline{3-5}
&	$\ \ \ \ + 125\ ,\invfb(\eminus_L\eminus_R) $&	merged &	120.065	$\pm$	0.088	&							\\ \hline

\end{tabular}
\caption{Resulting Higgs mass $\mH$ and cross sections $\sigma$ for the \emph{Model Independent Analysis} of the Higgs-Strahlung process for different leptonic final states and different options for sharing the luminosity $\mathcal{L}$.}
\label{tab:mirst}
\end{table}%

\begin{table}[!h]
\centering
\begin{tabular}{|l|c|l|l|l|}

\hline
Fit. &	Pol. &	Ch. &	$\mH$ (GeV) &	$\sigma$ (fb) \\ \hline
&	$\eminus_R\eplus_L$ &	$\mu\mu X$ &	119.951	$\pm$	0.084	&	6.98	$\pm$	0.45	(	6.45	\%)	\\ \cline{3-5}
&	$\mathcal{L}=250\ ,\invfb$ &	$eeX$ &	119.713	$\pm$	0.204	&	7.18	$\pm$	0.74	(	10.31	\%)	\\ \cline{3-5}
&	&	merged &	119.916	$\pm$	0.078	&							\\ \cline{2-5}
&	$\eminus_L\eplus_R$ &	$\mu\mu X$ &	119.905	$\pm$	0.077	&	10.26	$\pm$	0.55	(	5.36	\%)	\\ \cline{3-5}
 GPET &	$\mathcal{L}=250\ ,\invfb$ &	$eeX$ &	119.871	$\pm$	0.135	&	10.67	$\pm$	0.85	(	7.97	\%)	\\ \cline{3-5}
&	&	merged &	119.897	$\pm$	0.067	&							\\ \cline{2-5}
&	Joined &	$\mu\mu X$ &	119.926	$\pm$	0.080	&							\\ \cline{3-5}
&	$\mathcal{L}=$ $125\ ,\invfb(e^-_Re^+_L)$ &	$eeX$ &	119.823	$\pm$	0.159	&							\\ \cline{3-5}
&	$\ \ \ \ + 125\ ,\invfb(\eminus_L\eplus_R) $&	merged &	119.905	$\pm$	0.072	&							\\ \hline

&	$\eminus_R\eplus_L$ &	$\mu\mu X$ &	120.122	$\pm$	0.093	&	7.03	$\pm$	0.44	(	6.26	\%)	\\ \cline{3-5}
&	$\mathcal{L}=250\ ,\invfb$ &	$eeX$ &	119.689	$\pm$	0.204	&	7.23	$\pm$	0.74	(	10.24	\%)	\\ \cline{3-5}
&	&	merged &	120.047	$\pm$	0.085	&							\\ \cline{2-5}
&	$\eminus_L\eplus_R$ &	$\mu\mu X$ &	120.177	$\pm$	0.080	&	10.64	$\pm$	0.57	(	5.36	\%)	\\ \cline{3-5}
 CEG &	$\mathcal{L}=250\ ,\invfb$ &	$eeX$ &	120.053	$\pm$	0.149	&	10.67	$\pm$	0.85	(	7.97	\%)	\\ \cline{3-5}
&	&	merged &	120.149	$\pm$	0.070	&							\\ \cline{2-5}
&	Joined &	$\mu\mu X$ &	120.154	$\pm$	0.086	&							\\ \cline{3-5}
&	$\mathcal{L}=$ $125\ ,\invfb(\eminus_R\eplus_L)$ &	$eeX$ &	119.926	$\pm$	0.170	&							\\ \cline{3-5}
&	$\ \ \ \ + 125\ ,\invfb(\eminus_L\eplus_R) $&	merged &	120.108	$\pm$	0.077	&							\\ \hline

\end{tabular}
\caption{Resulting Higgs mass $\mH$ and cross section $\sigma$ for the \emph{Model Dependent Analysis} of the Higgs-Strahlung process for different leptonic final states and different options for sharing the luminosity $\mathcal{L}$.}
\label{tab:smrst}
\end{table}%

%\end{document}

